Short Non-Binary Low-Density Parity-Check Codes for Phase Noise Channels

This work considers the design of short non-binary low-density parity-check (LDPC) codes over finite fields of order m, for channels with phase noise. In particular, m-ary differential phase-shift keying (DPSK) modulated code symbols are transmitted over an additive white Gaussian noise (AWGN) channel with Wiener phase noise. At the receiver side, non-coherent detection takes place, with the help of a multi-symbol detection algorithm, followed by a non-binary decoding step. Both the detector and decoder operate on a joint factor graph. As a benchmark, finite length bounds and information rate expressions are computed and compared with the codeword error rate (CER) performance, as well as the iterative threshold of the obtained codes. As a result, performance within 1:2 dB from finite-length bounds is obtained, down to a CER of 1e-3.

==> iterative_detection_and_decoding.tex <==
\section{Iterative Detection and Decoding}
\label{sec:it_det_dec}

In the following, the structure of the receiver, which iteratively improves its estimate of the transmitted frames is explained. As also depicted in \fig{fig:receiver}, the channel samples $\rx$ are input to the detector together with apriori information regarding $\ismi{i}$, $\Ldai{i}=P(\ismi{i})$, which are \acp{p.m.f.} initially set to $[1/m,\ldots,1/m]$. The detector then produces extrinsic soft information $\Lde$ on the transmitted symbols $\ismi{i}$, $\Ldei{i} = P(\ismi{i}|\rx) / P(\ismi{i})$. Then the decoder computes in two steps from these apriori probabilities the extrinsic soft values $\Lce$: first $\Lcappi{i}\approx P(\cwi{i}|\Lcai{i})$ is computed by means of non-binary \ac{BP} and then $\Lce = \Lcappi{i} / \Lcai{i}$. Finally, this information is fed back to the detector, which computes a new estimate $\Ldei{i}$ with updated priors $\Lda$.


\begin{figure}[t]
	\centering	
	\includegraphics[scale=0.9]{figures/receiver}
	\caption{Structure of the iterative receiver. Still TODO: change location of Ls and add channel adapters}
	\label{fig:receiver}
\end{figure}


Also depicted in \fig{fig:receiver} are the two permutation blocks $\Pi(\cdot)$ and $\Pi^{-1}(\cdot)$. These are required first of all due to the use of the interleaver at the transmitter side and are inter-\ac{p.m.f.} permutations denoted by $\pi^{-1}(\cdot)$. 

Then, if channel adapters are used, each \ac{p.m.f.} $\Ldei{i}$ has to be permuted back as a function of the channel adapter value $\chadi{i}$ added to $\cwi{i}$. We denote this permutation by $\pi^{-1}_{\chadi{}}(\cdot)$ and note the fact that it is an intra-\ac{p.m.f.} permutation. 

Finally, by combining these two types of permutations, we obtain that $\Pi^{-1}=\pi^{-1}_{\chadi{}}\circ\pi^{-1}$.
Conversely, $\Pi=\pi_{\chadi{}}\circ\pi$, where the order in which the single permutations are performed does not play a role.

The structure of the detector is discussed in the following followed by a brief discussion on the decoder.

\subsection{Detection}

The role of the detector is to provide a \ac{MAP} estimate of the symbol-wise probability $P(\ismi{i}|\rx)$. Since only extrinsic information if forwarded to the decoder, this probability needs to be divided by the prior $P(\ismi{i})$, resulting in $\Ldei{i} = P(\ismi{i}|\rx) / P(\ismi{i})$. In order to compute these values, we start with $p(\ism, \boldsymbol{\psi}|\rx)$, which we factorize according to  
\begin{equation}
\label{eq::jointProb}
\begin{split}
p(\ism, \boldsymbol{\psi}|\rx) 
&= p(\rx|\ism,\boldsymbol{\psi}) p(\boldsymbol{\psi}|\ism) P(\ism) \frac{1}{p(\rx)}\\
&\propto p(\rxi{0}|\psi_0)\prod_{i = 1}^{N} p(\rxi{i}|\psi_i) p(\psi_i|\psi_{i-1}, \ismi{i}) P(\ismi{i})\,,
\end{split}
\end{equation}
where we have used the fact that due to the Wiener model and the differential modulation
$p(\psi_i|\psi_{i-1},\ldots,\psi_{0}, \ism)=p(\psi_i|\psi_{i-1},\ismi{i})$.
This factorization allows us to make use of factor graphs \cite{KFL01} and compute $P(\ismi{i}|\rx) / P(\ismi{i})$ as 

\begin{equation}
\label{eq::extrinsic}
%\begin{split}
\frac{P(\ismi{i}|\rx)}{P(\ismi{i})} =\int\displaylimits_{{0}}^{{2\pi}}\int\displaylimits_{{0}}^{{2\pi}}\alpha(\psi_{i-1})\beta(\psi_{i})p(\psi_{i}|\psi_{i-1}, \ismi{i})d\psi_id\psi_{i-1}
%\end{split}
\end{equation}
where $\alpha(\psi_i)$ and $\beta(\psi_i)$ are the forward/backward coefficients obtained from the factor graph as \cite{BC07}
\begin{equation}
\label{eq:fwd}
\begin{split}
\alpha(\psi_i) &= p(\rxi{i}|\psi_i)\cdot \\ & \quad \cdot \int\displaylimits_{0}^{2\pi} \left( \sum_{\ismi{i}} p(\psi_i|\psi_{i-1},\ismi{i})P(\ismi{i})\right) \alpha(\psi_{i-1}) \ d\psi_{i-1}
\end{split}
\end{equation}	
\begin{equation}
\begin{split}
\label{eq:bwd}
\beta&(\psi_i) = p(\rxi{i}|\psi_i) \cdot \\ &  \cdot\int\displaylimits_{0}^{2\pi} \left( \sum_{\ismi{i+1}} p(\psi_{i+1}|, \psi_i, \ismi{i+1})P(\ismi{i+1})\right) \beta(\psi_{i+1}) \ d\psi_{i+1} ,
\end{split}
\end{equation}
with $\alpha(\psi_0) = p(\rxi{0}|\psi_0)$ and $\beta(\psi_N)= p(\rxi{N}|\psi_N)$.

Next we elaborate on the expressions involved in the computation of the forward/backward coefficients. Firstly
\begin{equation}
p(\rxi{i}|\psi_i) = \frac{1}{\sqrt{2\pi\sigma^2}} e^{-\frac{|\rxi{i} - e^{j\psi_i}|^2}{2\sigma^2}}
\end{equation}

For the coherent case, where there is no phase uncertainty, i.e. $\theta_{i} = 0, \forall i$, in the above iteration the probability $p(\psi_i|\psi_{i-1}, \ismi{i})$ reduces to an indicator function 
\begin{equation}
p(\psi_i|\psi_{i-1}, \ismi{i}) \overset{\theta_i = 0}{=} \mathbbm{1}(e^{j\phi_i} = \ismi{i}e^{j\phi_{i-1}}) =
\begin{cases}
1, & \text{if}\ e^{j\phi_i} = \ismi{i}e^{j\phi_{i-1}}\\
0, &\text{otherwise}
\end{cases}.
\label{eq::indicator}
\end{equation}
and  the detector implements nothing else than the \ac{BCJR}\cite{BCJ+74} algorithm on the trellis of the differential modulator. 

For the non-coherent case we start with the Wiener model in \eqref{eq::wiener} and the identity $\phi_i =  \phi_{i-1} +\varphi_i$, which allows us to write $\psi_i = [\psi_{i-1} + \varphi_i + \Delta\theta_i]_{2\pi}$. Since $\ismi{i}=e^{j\varphi_i}$ is a deterministic mapping of  $\varphi{i}$, due to the modulation, it holds that
\begin{equation}
p(\psi_i|\psi_{i-1}, \ismi{i}) = p(\psi_i|\psi_{i-1}, \varphi_i) = p_\Delta (\psi_i - \psi_{i-1} - \varphi_{i})
\end{equation}
where $p_{\Delta}(\cdot)$ is the \ac{p.d.f.} of the phase increment $\Delta\theta_i$ in the Wiener process (modulo $2 \pi$). Furthermore, we can express
\begin{equation}
\label{eq:pDeltaInit}
p_\Delta (\varphi) = \sum\displaylimits_{\ell = -\infty}^{+\infty} g(0,\sigma_{\Delta}^{2};\varphi - 2\pi\ell)
\end{equation}
where
\begin{equation} \label{eq:normDistrg}
g(\mu,\sigma_{\Delta}^{2};\varphi) = \frac{1}{\sqrt{2\pi\sigma_{\Delta}^2}}e^{-\frac{(\varphi - \mu)^2}{2\sigma_{\Delta}^2}}\,.
\end{equation}
For practical values of $\sigma_\Delta$, the tails of the \ac{p.d.f.} in \eqref{eq:normDistrg} tend to zero in almost all points except some in the vicinity of $\mu$ \cite{BC11}, and we have that 
\begin{equation}
p_\Delta (\varphi) \simeq g(0,\sigma_{\Delta}^{2};\varphi)
\end{equation}
and thus \eqref{eq:pDeltaInit} simplifies to
\begin{equation} \label{eq:pDeltaFinal}
p_\Delta (\psi_i - \psi_{i-1} - \varphi_{i}) \simeq g(0,\sigma_{\Delta}^{2};\psi_i - \psi_{i-1} - \varphi_{i})\,.
\end{equation}

Even in its simplified form, using \eqref{eq:pDeltaFinal} in \eqref{eq::extrinsic}, \eqref{eq:fwd} and \eqref{eq:bwd} involves computing integrals of continuous \acp{p.d.f.}. A more practical approach is the use of a \ac{DP} algorithm \cite{Col13} which assumes $\psi_i$ only takes values in the discrete set $\{2\pi j/L\}$, $j\in\{ 0, \ldots, L - 1\}$, where $L$ is a design parameter. Combined with the fact that for practical values of $\sigma_{\Delta}$ the \ac{p.d.f.} in \eqref{eq:pDeltaFinal} has non-zero values only in the strict vicinity of 0, the following approximation \cite{PSG00} may be used 
\begin{equation}
p_\Delta(\varphi) =
\begin{cases}
1-P_\Delta, & \varphi=0\\
\frac{P_\Delta}{2}, &|\varphi|=\frac{2\pi}{L}\\
0, &\text{otherwise}
\end{cases}.
\label{eq::pDeltaDP}
\end{equation}
In accordance with \cite{PSG00}, a phase discretization factor of $L = 8 m$ has been chosen. The parameter $P_\Delta$ is a design parameter, also referred to in literature as transition probability of the discretized model \cite{BC11}. By using this approximation, the integrals in \eqref{eq::extrinsic}, \eqref{eq:fwd} and \eqref{eq:bwd} become summations and the computation of the forward/backward coefficients, as well as of the extrinsic probabilities becomes practical.


\subsection{Decoding}

Whereas decoding is concerned, we used for our system a standard non-binary \ac{LDPC} decoder, as explained in CITE. To reduce the complexity, we perform the check-node oprations in Fourier domain by using the Hadamard transform. We fix the internal number of iterations for the decoder to 1 and use external iterations with the detector to iteratively improve the estimate of the codeword symbols. 


